On the consistency of hyper-parameter selection in value-based deep reinforcement learning

Deep reinforcement learning (deep RL) has achieved tremendous success on various domains through a combination of algorithmic design and careful selection of hyper-parameters. Algorithmic improvements are often the result of iterative enhancements built upon prior approaches, while hyper-parameter choices are typically inherited from previous methods or fine-tuned specifically for the proposed technique. Despite their crucial impact on performance, hyper-parameter choices are frequently overshadowed by algorithmic advancements. This paper conducts an extensive empirical study focusing on the reliability of hyper-parameter selection for value-based deep reinforcement learning agents, including the introduction of a new score to quantify the consistency and reliability of various hyper-parameters. Our findings not only help establish which hyper-parameters are most critical to tune, but also help clarify which tunings remain consistent across different training regimes.

==> sections/environment_properties.tex <==
\section{Environment properties}
\label{sec:environment_properties}

The Arcade Learning Environment (ALE) is a platform designed for evaluating and comparing the performance of reinforcement learning algorithms on classic arcade games. ALE has emerged as the benchmark for evaluating the capabilities of reinforcement learning (RL) algorithms in tackling intricate discrete control tasks. Since its release in 2013 \citep{bellemare2012ale}, the benchmark has gained thousands of citations and almost all state-of-the-art RL algorithms have featured it in their work. However, results generated from the full benchmark have typically been limited to a few large research groups.

The cost of producing evaluations on the full dataset is not feasible for many researchers and not necessary if you want to evaluate some specific algorithm capabilities, like long context games. Therefore, here we provide some key properties of the environments based on our previous findings which will allow the RL community select a small but representative subsets of environments when evaluating specific algorithm capabilities.
